LABCAT: Locally adaptive Bayesian optimization using principal-component-aligned trust regions

Bayesian optimization (BO) is a popular method for optimizing expensive black-box functions. BO has several well-documented shortcomings, including computational slowdown with longer optimization runs, poor suitability for non-stationary or ill-conditioned objective functions, and poor convergence characteristics. Several algorithms have been proposed that incorporate local strategies, such as trust regions, into BO to mitigate these limitations; however, none address all of them satisfactorily. To address these shortcomings, we propose the LABCAT algorithm, which extends trust-region-based BO by adding a rotation aligning the trust region with the weighted principal components and an adaptive rescaling strategy based on the length-scales of a local Gaussian process surrogate model with automatic relevance determination. Through extensive numerical experiments using a set of synthetic test functions and the well-known COCO benchmarking software, we show that the LABCAT algorithm outperforms several state-of-the-art BO and other black-box optimization algorithms.

==> figures/Section4/coco_param_sweep/pprldmany_02D_hcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_param_sweep/pprldmany_02D_lcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_param_sweep/pprldmany_02D_mult2.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}}}


==> figures/Section4/coco_param_sweep/pprldmany_02D_multi.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}}}


==> figures/Section4/coco_param_sweep/pprldmany_02D_noiselessall.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}}}


==> figures/Section4/coco_param_sweep/pprldmany_02D_separ.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_param_sweep/pprldmany_03D_hcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_param_sweep/pprldmany_03D_lcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_param_sweep/pprldmany_03D_mult2.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_param_sweep/pprldmany_03D_multi.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_param_sweep/pprldmany_03D_noiselessall.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_param_sweep/pprldmany_03D_separ.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_param_sweep/pprldmany_05D_hcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algDperfprof}
\vfill \mbox{\algzeroperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_param_sweep/pprldmany_05D_lcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_param_sweep/pprldmany_05D_mult2.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}}}


==> figures/Section4/coco_param_sweep/pprldmany_05D_multi.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}}}


==> figures/Section4/coco_param_sweep/pprldmany_05D_noiselessall.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_param_sweep/pprldmany_05D_separ.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algEperfprof}}}


==> figures/Section4/coco_param_sweep/pprldmany_10D_hcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algzeroperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_param_sweep/pprldmany_10D_lcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_param_sweep/pprldmany_10D_mult2.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_param_sweep/pprldmany_10D_multi.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_param_sweep/pprldmany_10D_noiselessall.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_param_sweep/pprldmany_10D_separ.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/LABCAT noPC}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/LABCAT n10}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/LABCAT ULSP}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{final results/LABCAT p20}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_results/pprldmany_02D_hcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algMperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algNperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algLperfprof}
\vfill \mbox{\algIperfprof}
\vfill \mbox{\algGperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_results/pprldmany_02D_lcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algMperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algLperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algIperfprof}
\vfill \mbox{\algNperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algGperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_results/pprldmany_02D_mult2.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algMperfprof}
\vfill \mbox{\algLperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algNperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algBperfprof}
\vfill \mbox{\algGperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algIperfprof}}}


==> figures/Section4/coco_results/pprldmany_02D_multi.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algMperfprof}
\vfill \mbox{\algLperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algGperfprof}
\vfill \mbox{\algNperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algIperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_results/pprldmany_02D_noiselessall.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algMperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algLperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algNperfprof}
\vfill \mbox{\algIperfprof}
\vfill \mbox{\algGperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_results/pprldmany_02D_separ.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algMperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algLperfprof}
\vfill \mbox{\algIperfprof}
\vfill \mbox{\algNperfprof}
\vfill \mbox{\algGperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_results/pprldmany_03D_hcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_results/pprldmany_03D_lcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_results/pprldmany_03D_mult2.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_results/pprldmany_03D_multi.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_results/pprldmany_03D_noiselessall.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_results/pprldmany_03D_separ.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algFperfprof}
\vfill \mbox{\algzeroperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_results/pprldmany_05D_hcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algMperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algNperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algLperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algIperfprof}
\vfill \mbox{\algGperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_results/pprldmany_05D_lcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algMperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algNperfprof}
\vfill \mbox{\algLperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algIperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algGperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_results/pprldmany_05D_mult2.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algNperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algLperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algMperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algGperfprof}
\vfill \mbox{\algIperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_results/pprldmany_05D_multi.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algLperfprof}
\vfill \mbox{\algNperfprof}
\vfill \mbox{\algMperfprof}
\vfill \mbox{\algGperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algIperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_results/pprldmany_05D_noiselessall.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algMperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algNperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algLperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algIperfprof}
\vfill \mbox{\algGperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_results/pprldmany_05D_separ.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algMperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algNperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algLperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algGperfprof}
\vfill \mbox{\algIperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_results/pprldmany_10D_hcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algAperfprof}
\vfill \mbox{\algzeroperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algMperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algNperfprof}
\vfill \mbox{\algLperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algIperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_results/pprldmany_10D_lcond.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algMperfprof}
\vfill \mbox{\algNperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algLperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algIperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_results/pprldmany_10D_mult2.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algNperfprof}
\vfill \mbox{\algMperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algLperfprof}
\vfill \mbox{\algIperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_results/pprldmany_10D_multi.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algLperfprof}
\vfill \mbox{\algMperfprof}
\vfill \mbox{\algNperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algIperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_results/pprldmany_10D_noiselessall.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algMperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algNperfprof}
\vfill \mbox{\algLperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algIperfprof}
\vfill \mbox{\algBperfprof}}}


==> figures/Section4/coco_results/pprldmany_10D_separ.tex <==
\providecommand{\nperfprof}{7}\providecommand{\algAperfprof}{\StrLeft{final results/LABCAT}{\nperfprof}}\providecommand{\algBperfprof}{\StrLeft{final results/random}{\nperfprof}}\providecommand{\algCperfprof}{\StrLeft{final results/turbo1 2d+1}{\nperfprof}}\providecommand{\algDperfprof}{\StrLeft{final results/BADS}{\nperfprof}}\providecommand{\algEperfprof}{\StrLeft{final results/EGO}{\nperfprof}}\providecommand{\algFperfprof}{\StrLeft{2017/DTS-CMA-ES Pitra}{\nperfprof}}\providecommand{\algGperfprof}{\StrLeft{final results/TREGO incomp}{\nperfprof}}\providecommand{\algHperfprof}{\StrLeft{2009/MCS huyer noiseless}{\nperfprof}}\providecommand{\algIperfprof}{\StrLeft{final results/SRSM}{\nperfprof}}\providecommand{\algJperfprof}{\StrLeft{2009/NEWUOA ros noiseless}{\nperfprof}}\providecommand{\algKperfprof}{\StrLeft{2013/SMAC-BBOB hutter noiseless}{\nperfprof}}\providecommand{\algLperfprof}{\StrLeft{final results/turbo5 2d+1}{\nperfprof}}\providecommand{\algMperfprof}{\StrLeft{final results/AutoSAEA}{\nperfprof}}\providecommand{\algNperfprof}{\StrLeft{final results/trlbo 2d+1}{\nperfprof}}\providecommand{\algzeroperfprof}{best 2009}\providecommand{\perfprofsidepanel}{{\mbox{\algzeroperfprof}
\vfill \mbox{\algFperfprof}
\vfill \mbox{\algDperfprof}
\vfill \mbox{\algHperfprof}
\vfill \mbox{\algMperfprof}
\vfill \mbox{\algNperfprof}
\vfill \mbox{\algAperfprof}
\vfill \mbox{\algJperfprof}
\vfill \mbox{\algLperfprof}
\vfill \mbox{\algCperfprof}
\vfill \mbox{\algKperfprof}
\vfill \mbox{\algIperfprof}
\vfill \mbox{\algEperfprof}
\vfill \mbox{\algBperfprof}}}

